Diffusion Models as Data Mining Tools

This paper demonstrates how to use generative models trained for image synthesis as tools for visual data mining. Our insight is that since contemporary generative models learn an accurate representation of their training data, we can use them to summarize the data by mining for visual patterns. Concretely, we show that after finetuning conditional diffusion models to synthesize images from a specific dataset, we can use these models to define a typicality measure on that dataset. This measure assesses how typical visual elements are for different data labels, such as geographic location, time stamps, semantic labels, or even the presence of a disease. This analysis-by-synthesis approach to data mining has two key advantages. First, it scales much better than traditional correspondence-based approaches since it does not require explicitly comparing all pairs of visual elements. Second, while most previous works on visual data mining focus on a single dataset, our approach works on diverse datasets in terms of content and scale, including a historical car dataset, a historical face dataset, a large worldwide street-view dataset, and an even larger scene dataset. Furthermore, our approach allows for translating visual elements across class labels and analyzing consistent changes.

==> figures/clusters/cars.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}{0.23\linewidth}
        \centering
        \includegraphics[width=\textwidth]{images/cars/1920s.png}
        \caption{\textbf{1920s}}
        \label{cluster:car:20}
    \end{subfigure}
    \begin{subfigure}{0.23\linewidth}
        \includegraphics[width=\textwidth]{images/cars/1930s.png}
        \caption{\textbf{1930s}}
        \label{cluster:car:30}
    \end{subfigure}
    \begin{subfigure}{0.23\linewidth}
        \vspace{0.5em}
        \includegraphics[width=\textwidth]{images/cars/1940s.png}
        \caption{\textbf{1940s}}
        \label{cluster:car:40}
    \end{subfigure}
    \begin{subfigure}{0.23\linewidth}
        \includegraphics[width=\textwidth]{images/cars/1950s.png}
        \caption{\textbf{1950s}}
        \label{cluster:car:50}
    \end{subfigure}
    \begin{subfigure}{0.23\linewidth}
        \includegraphics[width=\textwidth]{images/cars/1960s.png}
        \caption{\textbf{1960s}}
        \label{cluster:car:60}
    \end{subfigure}
    \begin{subfigure}{0.23\linewidth}
        \includegraphics[width=\textwidth]{images/cars/1970s.png}
        \caption{\textbf{1970s}}
        \label{cluster:car:70}
    \end{subfigure}
    \begin{subfigure}{0.23\linewidth}
        \includegraphics[width=\textwidth]{images/cars/1980s.png}
        \caption{\textbf{1980s}}
        \label{cluster:car:80}
    \end{subfigure}
    \begin{subfigure}{0.23\linewidth}
        \includegraphics[width=\textwidth]{images/cars/1990s.png}
        \caption{\textbf{1990s}}
        \label{cluster:car:90}
    \end{subfigure}
    \caption{\textbf{Mining typical car elements across decade.} Using our measure of typicality we can rank and cluster visual elements that characterize cars across century using the CarDB dataset \cite{cardb}. During clustering we append DIFT-61 \cite{dift} of our finetuned model to the existing CLIP-features to enforce correspondence. For each decade, we show the first 6 images from 4 clusters out of 30 in ranking order of typicallity. \ys{maybe add some analysis}}
    \label{fig:clusters}
\end{figure*}

==> figures/clusters/faces.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\textwidth]{images/faces/1940.png}
        \caption{\textbf{1940s}}
        \label{cluster:car:20}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=\textwidth]{images/faces/1950.png}
        \caption{\textbf{1950s}}
        \label{cluster:car:30}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \vspace{0.5em}
        \includegraphics[width=\textwidth]{images/faces/1960.png}
        \caption{\textbf{1960s}}
        \label{cluster:car:40}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=\textwidth]{images/faces/1970.png}
        \caption{\textbf{1970s}}
        \label{cluster:car:50}
    \end{subfigure}
    \caption{\textbf{Mining typical faces elements between decades.} Using our measure of typicality we can rank and cluster visual elements that characterize faces across decades on the dataset of Faces Through Time \cite{ftt}. Here, we contrast the typicality measure not only with the unconditional but also with the previous and next decade. For each decade, we show the first 5 images from 4 top ranked clusters out of 30 ranked in order of typicality. \ys{maybe add some analysis - I have a huge hang time on my cluster - I noticed finetuning models improves results both here and in the case of cars}}
    \label{fig:clusters}
\end{figure*}

==> figures/clusters/geo.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=\textwidth]{images/clusters/Frame 26.png}
        \caption{\textbf{United States}}
        \label{cluster:us}
    \end{subfigure}\hspace{1em}
    \begin{subfigure}{0.48\linewidth}
    \includegraphics[width=\textwidth]{images/clusters/russian-clusters 1.png}
    \caption{\textbf{Russia}}
    \label{cluster:russia}
    \end{subfigure}
    \begin{subfigure}{0.48\linewidth}
    \vspace{0.5em}
    \includegraphics[width=\textwidth]{images/clusters/nigeria-clusters 1.png}
    \caption{\textbf{Nigeria}}
    \label{cluster:nigeria}
    \end{subfigure}\hspace{1em}
    \begin{subfigure}{0.48\linewidth}
    \includegraphics[width=\textwidth]{images/clusters/uk-clusters-reorder 1.png}
    \caption{\textbf{United Kingdom}
    % The characteristic chimneys summarizing the whole modern history of the UK.
    }
    \label{cluster:uk}
    \end{subfigure}
    \caption{\textbf{Clustering visual elements typical for a specific country.} Using our measure of typicality we can rank and cluster visual elements that characterize each country. For each country, we show images from 6 clusters out of 32. (a) US: large cars, windows, stop signs, road marks and post boxes; (b) Russia: multi-colored dachas, khrushchevkas, electricity poles (upper \& lower) and silver birch trees; (c) Nigeria: (palm or neem) trees, triangle roofs \& arches, electricity poles, busy streets, striped pavement edges; (d) UK: chimneys, white  windows on brick walls, black roofs, roof pipes and yellow license plates.}
    \label{fig:clusters}
\end{figure*}

==> figures/compare.tex <==
\def\topkalllen{0.29}

\begin{figure}[]
    \centering
    \hspace{-4pt}

    \begin{subfigure}{0.3 \textwidth}
        \centering
        % \makebox[7pt]{\hspace{-15pt}\raisebox{3pt}{$\typicality$}}
        \includegraphics[width=\textwidth]{images/compare/cars/0.png}
        % \makebox[7pt]{\hspace{-18pt}\raisebox{3pt}{Rand.}}
        \includegraphics[width=\textwidth]{images/compare/cars/1.png}
        % \makebox[7pt]{\hspace{-23pt}\raisebox{3pt}{$-\typicality$}}
        \includegraphics[width=\textwidth]{images/compare/cars/2.png}
        \vspace{1pt}
        \caption{\textbf{CarDB} \cite{cardb}}
        \label{topkfull:cars}
    \end{subfigure}

    \begin{subfigure}{0.9 \textwidth}
        \centering

        \caption{\textbf{FTT} \cite{ftt}}
        \label{topkfull:faces}
    \end{subfigure}

    \begin{subfigure}{0.9 \textwidth}
        \centering

        \label{topkfull:geo}
        \caption{$G^3$ \cite{cardb}}
    \end{subfigure}
    
    \caption{\textbf{Total typicality ranking.} We visualize the top-5 images for 2 classes from each of the 3 different datasets: (a) CarDB: \topkcarsa (top), \topkcarsb (bottom). (b) FTT: \topkftta (top), \topkfttb (bottom). (c) $G^3$: \topkgeoa (top) , \topkgeob (bottom). The patches are ranked according to typicality ($\typicality$) according to negative typicality ($-\typicality$), and randomly (Rand.). 
}
    \label{fig:topk:full}
\end{figure}

==> figures/finetuning/thailand.tex <==
\begin{figure}
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=165px]{images/finetuning/thailand/before.png}
        \caption{Stable Diffusion (V15)}
    \end{subfigure}
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=165px]{images/finetuning/thailand/after.png}
        \caption{Stable Diffusion finetuned on $G^3$ \cite{g3}}
    \end{subfigure}
    \label{fig:finetuning-qualitative}
    \caption{\textbf{Effect of finetuning (qualitative)}. Except from the effect of focusing the typicality score as shown in Figure \label{fig:finetuning-quantitative}, finetuning also allows the model to change the elements that are considered most typical. In this example we demonstrate the top-10 clusters according to average ranking where the baseline model of Stable Diffusion focuses on cultural elements of the Thai landscape, such as temples, motorbikes, and trees, whereas the finetuned model prioritizes electricity poles, common architectural materials, road tracks, lamp posts bollards and even stitching artifacts. By visualizin the typicallity overlayed onto the images we can observe that the model pays attention to details in both cases hence this is not the result of noisy predictions.}
\end{figure}



==> figures/general-amb.tex <==
\def\topkalllen{0.98}

\begin{figure}[!ht]
    \centering
    \hspace{-4pt}

    \begin{subfigure}{\topkalllen \textwidth}
        \centering
        \makebox[7pt]{\hspace{-15pt}\raisebox{20pt}{$\typicality$}}\includegraphics[width=0.9\textwidth]{images/best-images/cars_1930_D.png}
        \makebox[7pt]{\hspace{-20pt}\raisebox{20pt}{Rand.}}\includegraphics[width=0.9\textwidth]{images/best-images/cars_1930_random.png}
        \makebox[7pt]{\hspace{-16pt}\raisebox{20pt}{$-\typicality$\hspace{4pt}}}\includegraphics[width=0.9\textwidth]{images/best-images/cars_1930_D_least.png}
        \vspace{0.5pt}
        \caption{\textbf{CarDB} \cite{cardb}}
        \label{topkfull:cars}
        \vspace{0.5pt}
    \end{subfigure}
    \vspace{0.5pt}
    \begin{subfigure}{\topkalllen \textwidth}
        \centering
        \makebox[7pt]{\hspace{-15pt}\raisebox{20pt}{$\typicality$}}\includegraphics[width=0.9\textwidth]{images/best-images/1970_D.png}
        \makebox[7pt]{\hspace{-18pt}\raisebox{20pt}{Rand.}}\includegraphics[width=0.9\textwidth]{images/best-images/1970_random.png}
        \makebox[7pt]{\hspace{-23pt}\raisebox{20pt}{\hspace{4pt}$-\typicality$}}\includegraphics[width=0.9\textwidth]{images/best-images/1970_D_least.png}
        \vspace{0.5pt}
        \caption{\textbf{FTT} \cite{ftt}}
        \label{topkfull:faces}
        \vspace{0.5pt}
    \end{subfigure}
    \vspace{0.5pt}
    \begin{subfigure}{\topkalllen \textwidth}
        \centering
        \makebox[7pt]{\hspace{-15pt}\raisebox{20pt}{$\typicality$}}\includegraphics[width=0.9\textwidth]{images/best-images/Japan_D.png}
        \makebox[7pt]{\hspace{-18pt}\raisebox{20pt}{Rand.}}\includegraphics[width=0.9\textwidth]{images/best-images/Japan_random.png}
        \makebox[7pt]{\hspace{-16pt}\raisebox{20pt}{$-\typicality$\hspace{4pt}}}\includegraphics[width=0.9\textwidth]{images/best-images/Japan_D_least.png}
        \vspace{0.5pt}
        \caption{$G^3$ \cite{cardb}}
        \label{topkfull:geo}
        \vspace{0.5pt}
    \end{subfigure}
    
    \caption{\textbf{Total typicality ranking.} We visualize the top-5 images according to average $\typicality$, $-\typicality$, and random order, for one class of CarDB (1930s), FTT (1970s) and $G^3$ (Japan). 
}
    \label{fig:topk:full}
\end{figure}

==> figures/parallel-dataset.tex <==
\newcommand{\highlight}[1]{\tikz[baseline=(X.base)]{\node[draw=red,rectangle,fill=red!20,rounded corners,inner sep=2pt] (X) {#1};}}

\begin{table*}[!ht]
  \centering
   \setlength{\tabcolsep}{0pt} % Remove horizontal padding
  \renewcommand{\arraystretch}{0} % Remove vertical padding
  % \begin{adjustbox}{width=1.0\textwidth} % Scale the table to fit the page width
      \begin{tabular}{cccccccccc}
        USA & Japan & France & Italy & UK & Brazil & Russia & Thailand & Nigeria & India \\
        % \hline
        \highlight{\includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/US/64821_United States.jpeg}} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/US/64821_Japan.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/US/64821_France.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/US/64821_Italy.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/US/64821_United Kingdom.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/US/64821_Brazil.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/US/64821_Russia.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/US/64821_Thailand.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/US/64821_Nigeria.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/US/64821_India.jpeg} \\
        \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Japan/250888_United States.jpeg} & \highlight{\includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Japan/250888_Japan.jpeg}} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Japan/250888_France.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Japan/250888_Italy.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Japan/250888_United Kingdom.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Japan/250888_Brazil.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Japan/250888_Russia.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Japan/250888_Thailand.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Japan/250888_Nigeria.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Japan/250888_India.jpeg} \\
         \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/France/154662_United States.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/France/154662_Japan.jpg} & \highlight{\includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/France/154662_France.jpg}} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/France/154662_Italy.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/France/154662_United Kingdom.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/France/154662_Brazil.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/France/154662_Russia.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/France/154662_Thailand.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/France/154662_Nigeria.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/France/154662_India.jpg} \\
        % Repeat similar lines for the remaining rows
        \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Italy/260760_United States.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Italy/260760_Japan.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Italy/260760_France.jpeg} & \highlight{\includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Italy/260760_Italy.jpeg}} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Italy/260760_United Kingdom.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Italy/260760_Brazil.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Italy/260760_Russia.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Italy/260760_Thailand.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Italy/260760_Nigeria.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Italy/260760_India.jpeg} \\
         \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/UK/179015_United States.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/UK/179015_Japan.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/UK/179015_France.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/UK/179015_Italy.jpeg} & \highlight{\includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/UK/179015_United Kingdom.jpeg}} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/UK/179015_Brazil.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/UK/179015_Russia.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/UK/179015_Thailand.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/UK/179015_Nigeria.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/UK/179015_India.jpeg} \\
        \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Brazil/6129_United States.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Brazil/6129_Japan.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Brazil/6129_France.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Brazil/6129_Italy.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Brazil/6129_United Kingdom.jpg} & \highlight{\includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Brazil/6129_Brazil.jpg}} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Brazil/6129_Russia.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Brazil/6129_Thailand.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Brazil/6129_Nigeria.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Brazil/6129_India.jpg} \\
         \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Russia/286470_United States.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Russia/286470_Japan.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Russia/286470_France.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Russia/286470_Italy.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Russia/286470_United Kingdom.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Russia/286470_Brazil.jpg} & \highlight{\includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Russia/286470_Russia.jpg}} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Russia/286470_Thailand.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Russia/286470_Nigeria.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Russia/286470_India.jpg} \\
         \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Thailand/220951_United States.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Thailand/220951_Japan.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Thailand/220951_France.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Thailand/220951_Italy.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Thailand/220951_United Kingdom.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Thailand/220951_Brazil.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Thailand/220951_Russia.jpg} & \highlight{\includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Thailand/220951_Thailand.jpg}} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Thailand/220951_Nigeria.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Thailand/220951_India.jpg} \\
         \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Nigeria/24544_United States.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Nigeria/24544_Japan.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Nigeria/24544_France.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Nigeria/24544_Italy.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Nigeria/24544_United Kingdom.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Nigeria/24544_Brazil.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Nigeria/24544_Russia.jpg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Nigeria/24544_Thailand.jpg} & \highlight{\includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Nigeria/24544_Nigeria.jpg}} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/Nigeria/24544_India.jpg} \\
         \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/India/200033_United States.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/India/200033_Japan.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/India/200033_France.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/India/200033_Italy.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/India/200033_United Kingdom.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/India/200033_Brazil.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/India/200033_Russia.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/India/200033_Thailand.jpeg} & \includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/India/200033_Nigeria.jpeg} & \highlight{\includegraphics[width=0.092\textwidth]{images/parallel-ranked-1/India/200033_India.jpeg}} \\
      \end{tabular}
      \captionof{figure}{\textbf{Parallel Dataset.} Real images (highlighted in {{red}}) are transposed across multiple locations using Plug and Play \cite{tumanyan2023plug}, showing an overall preservation of semantic layout and content. For more translated images, see the submitted webpage.
      }
      \label{fig:parallel}
  % \end{adjustbox} % Scale the table to fit the page width
\end{table*}


==> figures/stats.tex <==
\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \centering
        \begin{minipage}[b]{0.3\textwidth}
            \centering
            \includegraphics[width=5.33em]{images/trans/gt.png}
            \par\noindent
            \tiny
            Original
        \end{minipage}
        \begin{minipage}[b]{0.3\textwidth}
            \centering
            \includegraphics[width=5.33em]{images/trans/sd-v15.png}
            \par\noindent
            \tiny
            Pretrained
        \end{minipage}
        \begin{minipage}[b]{0.3\textwidth}
            \centering
            \includegraphics[width=5.33em]{images/trans/ft.png}
            \par\noindent
            \tiny
            Finetuned
        \end{minipage}
        \caption{Effect of finetuning on the parallel dataset.}
        \label{fig:ftparallel}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \begin{minipage}[b]{0.2\textwidth}
            \centering
            \includegraphics[width=4.25em]{images/stats/car.png}
            \par\noindent
            \tiny
            Car
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.2\textwidth}
            \centering
            \includegraphics[width=4.25em]{images/stats/dirt.png}
            \par\noindent
            \tiny
            Dirt Road
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.2\textwidth}
            \centering
            \includegraphics[width=4.25em]{images/stats/person.png}
            \par\noindent
            \tiny
            Person
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.2\textwidth}
            \centering
            \includegraphics[width=4.25em]{images/stats/potted plant.png}
            \par\noindent
            \tiny
            Plant Pots
        \end{minipage}
        \caption{Quantitative analysis and comparison.}
        \label{fig:stats}
    \end{subfigure}
    
    \caption{\textbf{Generating a parallel dataset.} Analyzing the translation of images from one country to another using Plug and Play \cite{tumanyan2023plug} becomes only possible after finetuning \update{(e.g., France to Thailand; Fig.~\ref{fig:ftparallel})}. A quantitative analysis of \update{generic} statistical differences using a segmentation network (Fig.~\ref{fig:stats}) on \update{our} parallel dataset reveals certain trends for
    \textcolor[rgb]{0.12156863, 0.46666667, 0.70588235}{\textbf{USA}},
\textcolor[rgb]{1, 0.49803922, 0.05490196}{\textbf{Japan}},
\textcolor[rgb]{0.17254902, 0.62745098, 0.17254902}{\textbf{France}},
\textcolor[rgb]{0.83921569, 0.15294118, 0.15686275}{\textbf{Italy}},
\textcolor[rgb]{0.58039216, 0.40392157, 0.74117647}{\textbf{UK}},
\textcolor[rgb]{0.76862745, 0.61176471, 0.58039216}{\textbf{Brazil}},
\textcolor[rgb]{0.96862745, 0.71372549, 0.82352941}{\textbf{Russia}},
\textcolor[rgb]{0.78039216, 0.78039216, 0.78039216}{\textbf{Thailand}},
\textcolor[rgb]{0.85882353, 0.85882353, 0.55294118}{\textbf{Nigeria}}, and 
\textcolor[rgb]{0.61960784, 0.85490196, 0.89803922}{\textbf{India}}, yet \update{can't showcase dataset specific visual differences (e.g., of road line color or style).}
}
\label{generating-pd}
\vspace{-0.5em}
\end{figure}


==> figures/topk.tex <==
\begin{figure*}
    \centering
    \hspace{4pt}
    \begin{subfigure}{0.31\textwidth}
        \centering
        \makebox[7pt]{\hspace{-15pt}\raisebox{7pt}{$\typicality$}}\includegraphics[trim={0 0 12540 0}, clip, width=\textwidth]{images/topk/D/United States.png}
        \makebox[7pt]{\hspace{-15pt}\raisebox{7pt}{$\tbar$}}\includegraphics[trim={0 0 12540 0}, clip, width=\textwidth]{images/topk/D_bar/United States.png}
        \makebox[7pt]{\hspace{-18pt}\raisebox{7pt}{Rand.}}\includegraphics[trim={0 0 12540 0}, clip, width=\textwidth]{images/topk/random/United States.png}
        \makebox[7pt]{\hspace{-23pt}\raisebox{7pt}{$-\typicality$}}\includegraphics[trim={0 0 0 0}, clip, 
        width=\textwidth]{images/topk/D_least/us-d.png}
        \makebox[7pt]{\hspace{-23pt}\raisebox{7pt}{$-\tbar$}}\includegraphics[trim={0 0 0 0}, clip, width=\textwidth]{images/topk/D_bar_least/us-dbar.png}
        \label{topk:us}
        \vspace{-0.9em}
        \caption{\textbf{United States}}
    \end{subfigure}
    \hspace{5pt}
    \begin{subfigure}{0.31\linewidth}
        \includegraphics[trim={0 0 12540 0}, clip, width=\textwidth]{images/topk/D/Russia.png}
        \includegraphics[trim={0 0 12540 0}, clip, width=\textwidth]{images/topk/D_bar/Russia.png}
        \includegraphics[trim={0 0 12540 0}, clip, width=\textwidth]{images/topk/random/Russia.png}
        \includegraphics[trim={0 0 0 0}, clip, 
        width=\textwidth]{images/topk/D_least/russia-d.png}
        \includegraphics[trim={0 0 0 0}, clip, width=\textwidth]{images/topk/D_bar_least/russia-fix.png}
        \label{topk:russia}
        \vspace{-0.9em}
        \caption{\textbf{Russia}}
    \end{subfigure}
    \begin{subfigure}{0.31\textwidth}
        \centering
        \includegraphics[trim={0 0 12540 0}, clip, width=\textwidth]{images/topk/D/Italy.png}
        \includegraphics[trim={0 0 12540 0}, clip, width=\textwidth]{images/topk/D_bar/Italy.png}
        \includegraphics[trim={0 0 12540 0}, clip, width=\textwidth]{images/topk/random/Italy.png}
        \includegraphics[trim={0 0 12540 0}, clip, 
        width=\textwidth]{images/topk/D_least/Italy.png}
        \includegraphics[trim={0 0 0 0}, clip, width=\textwidth]{images/topk/D_bar_least/italy-dbar.png}
        \label{cluster:italy}
        \vspace{-0.9em}
        \caption{\textbf{Italy}}
    \end{subfigure}
    \vspace{-0.7em}
    \caption{\textbf{Typicality measures.} We visualize the top-7 patches for 3 countries (US, Russia and Italy) ranked according to typicality ($\typicality$), according to cross location-typicality ($\tbar$), randomly (Rand.), according to inverse typicality ($-\typicality$), and according to inverse cross-location typicality ($-\tbar$). %We manually remove constant color images, which correspond to clouds and are highly non-co-typical..
}
    \label{fig:topk}
\end{figure*}

==> operational-figures/finetuning-supmat.tex <==
\begin{figure}[!ht]
    \centering
    \begin{subfigure}{0.43\textwidth}
        \centering
        \includegraphics[width=\textwidth]{operational-images-supmat/cars/pt/clusters/ranked/dift-161/32/1960__hard_limit_7__top_k_7__min_im_6.png}
        \includegraphics[width=\textwidth]{operational-images-supmat/faces/pt/clusters/random/dift-161/32/1880__hard_limit_7__top_k_7__min_im_6.png}
        \includegraphics[width=\textwidth]{operational-images-supmat/geo/pt/clusters/ranked/clip/32/Thailand__hard_limit_7__top_k_7__min_im_6.png}

        \caption{\textbf{Stable Diffusion (V1.5)}}
    \end{subfigure}
    \hspace{1em}
    \begin{subfigure}{0.43\textwidth}
        \centering
        \includegraphics[width=\textwidth]{operational-images-supmat/cars/ft/clusters/ranked/dift-161/32/1960__hard_limit_7__top_k_7__min_im_6.png}
        \includegraphics[width=\textwidth]{operational-images-supmat/faces/ft/clusters/ranked/dift-161/32/1880__hard_limit_7__top_k_7__min_im_6.png}
        \includegraphics[width=\textwidth]{operational-images-supmat/geo/ft/clusters/ranked/clip/32/Thailand__hard_limit_7__top_k_7__min_im_6.png}
        \caption{\textbf{Finetuned}}
    \end{subfigure}

    \caption{\textbf{Top-7 Cluster before and after finetuning}. We show results in 3 different datasets CarDB (1960) \cite{cardb}, FTT (1880) \cite{ftt}, and $G^3$ (Thailand) \cite{g3}. **See text for details.}
    \label{fig:finetuning-qualitative}
\end{figure}

==> operational-figures/finetuning.tex <==
\begin{figure}
    \centering
    \begin{subfigure}{0.20\textwidth}
        \includegraphics[width=\textwidth,height=5.3cm]{images/14.png}
    \end{subfigure}
    % \includegraphics[width=0.2\textwidth]{images/compare/cars/2.png}
    % \includegraphics[width=0.1\textwidth]{images/compare/cars/3.png}
    \begin{subfigure}{0.145\textwidth}
        \includegraphics[width=\textwidth,height=5.3cm]{images/384.png}
    \end{subfigure}
    \begin{subfigure}{0.145\textwidth}
        \includegraphics[width=\textwidth,height=5.3cm]{images/716.png}
    \end{subfigure}
    % \includegraphics[width=0.05\textwidth]{images/compare/faces/6.png}
    % \includegraphics[width=0.2\textwidth]{images/compare/geo/0.png}
   \begin{subfigure}{0.23\textwidth}
       \includegraphics[width=\textwidth,height=5.3cm]{images/34.png}
    \end{subfigure}
   \begin{subfigure}{0.23\textwidth}
       \includegraphics[width=\textwidth, height=5.3cm]{images/113.png}
    \end{subfigure}
    % \includegraphics[width=0.1\textwidth]{images/compare/geo/24.png}
    \caption{\textbf{Effect of finetuning}. \update{Using examples} from our three datasets (CarDB \cite{cardb}, FTT \cite{ftt}, and $G^3$ \cite{g3}), we show \update{how} for different images (top row) the regions with high typicality \update{change} before (middle row) and after (bottom row) fine-tuning. Notice how typicality changes from almost random elements before fine-tuning to the most typical ones after fine-tuning, especially for the $G^3$ data.
    }
    \label{fig:finetuning-qualitative}
    \vspace{-1em}
\end{figure}


